Generative Motion Stylization of Cross-structure Characters within Canonical Motion Space

Stylized motion breathes life into characters. However, the fixed skeleton structure and style representation hinder existing data-driven motion synthesis methods from generating stylized motion for various characters. In this work, we propose a generative motion stylization pipeline, named MotionS, for synthesizing diverse and stylized motion on cross-structure characters using cross-modality style prompts. Our key insight is to embed motion style into a cross-modality latent space and perceive the cross-structure skeleton topologies, allowing for motion stylization within a canonical motion space. Specifically, the large-scale Contrastive-Language-Image-Pre-training (CLIP) model is leveraged to construct the cross-modality latent space, enabling flexible style representation within it. Additionally, two topology-encoded tokens are learned to capture the canonical and specific skeleton topologies, facilitating cross-structure topology shifting. Subsequently, the topology-shifted stylization diffusion is designed to generate motion content for the particular skeleton and stylize it in the shifted canonical motion space using multi-modality style descriptions. Through an extensive set of examples, we demonstrate the flexibility and generalizability of our pipeline across various characters and style descriptions. Qualitative and quantitative comparisons show the superiority of our pipeline over state-of-the-arts, consistently delivering high-quality stylized motion across a broad spectrum of skeletal structures.

==> sections/figures.tex <==
\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=1.0\linewidth]{figures/exp1.pdf}
\end{center}
   \caption{\textbf{Qualitative comparison with SinMDM.} SinMDM$^{*}$ refers to the model that is trained on the source motion instead of the style motion. Motion$\mathbb{S}$ effectively handles various skeleton structures, stylizing the source motion based on key features of multi-modality style prompts. However, SinMDM exhibits unstable performance in expressing both the motion content and style.}
\label{fig:exp1}
\end{figure*}

\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=1.0\linewidth]{figures/exp2.pdf}
\end{center}
   \caption{\textbf{Qualitative comparison with DME and MotionPuzzle.} The results of Motion$\mathbb{S}$ are realistic, while the results of DME and MotionPuzzle suffer from motion distortion when complex style prompts are used.}
\label{fig:exp2}
\end{figure*}


\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=0.95\linewidth]{figures/exp3.pdf}
\end{center}
   \caption{\textbf{Qualitative ablation study.} The proposed cross-modality style embedding and cross-structure topology shifting strategies are both effective and collaborate to construct the canonical motion space, resulting in high-quality stylized results. }
\label{fig:exp3}
\end{figure*}

\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=1.0\linewidth]{figures/exp4.pdf}
\end{center}
   \caption{\textbf{Evaluation of the generalizability.} Our Motion$\mathbb{S}$ achieves zero-shot style control using unseen style prompts.}
\label{fig:exp4}
\end{figure*}

\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=0.9\linewidth]{figures/exp5.pdf}
\end{center}
   \caption{\textbf{Evaluation of the generative stylization.} Motion$\mathbb{S}$ can generate diverse stylized motion from a single content sequence, a capability not achieved by existing motion stylization methods.}
\label{fig:exp5}
\end{figure*}


\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=1.0\linewidth]{figures/exp6.pdf}
\end{center}
   \caption{\textbf{Application of the linear interpolation weight $\alpha$ in inference.} Manually adjusting $\alpha$ can obtain smooth motion stylization.}
\label{fig:exp6}
\end{figure*}


\begin{figure*}[t]
% \vspace{-.2cm}
% \setlength{\abovecaptionskip}{-.1cm}
% \setlength{\belowcaptionskip}{-.3cm}
\begin{center}
   \includegraphics[width=0.9\linewidth]{figures/exp7.pdf}
\end{center}
   \caption{\textbf{Application in text-based motion editing.} We train the TSD on a text-to-motion dataset and assess our Motion$\mathbb{S}$' performance in motion editing.}
\label{fig:exp7}
\end{figure*}
